Reinforced Medical Report Generation with X-Linear Attention and Repetition Penalty

To reduce doctors' workload, deep-learning-based automatic medical report generation has recently attracted more and more research efforts, where attention mechanisms and reinforcement learning are integrated with the classic encoder-decoder architecture to enhance the performance of deep models. However, these state-of-the-art solutions mainly suffer from two shortcomings: (i) their attention mechanisms cannot utilize high-order feature interactions, and (ii) due to the use of TF-IDF-based reward functions, these methods are fragile with generating repeated terms. Therefore, in this work, we propose a reinforced medical report generation solution with x-linear attention and repetition penalty mechanisms (ReMRG-XR) to overcome these problems. Specifically, x-linear attention modules are used to explore high-order feature interactions and achieve multi-modal reasoning, while repetition penalty is used to apply penalties to repeated terms during the model's training process. Extensive experimental studies have been conducted on two public datasets, and the results show that ReMRG-XR greatly outperforms the state-of-the-art baselines in terms of all metrics.

==> Conclusion.tex <==

	\section{Conclusion and Future Work}
	
	In this paper, we have proposed to use x-linear attention, which integrates bi-linear pooling to explore high-order feature interactions for intra-modal and inter-modal reasoning, for medical report generation. We have also used reinforcement learning with diversity to generate long paragraphs. We have conducted extensive experiments on two publicly available datasets, IU X-Ray and MIMIC-CXR, which have demonstrated the superior performance of our proposed approach to achieve state-of-the-art results.
	
%		While our ReMRG-XR method for medical report generation has achieved  superior performance compared to other state-of-the-art works, its performance could be further improved in the future by dealing with the following  challenges.
		As there is no effective metrics especially designed for medical report generation, to evaluate our generated results more effectively, we will explore a more reasonable and effective metric	for medical report generation in future work. 
		Most current works utilizing reinforcement learning only optimize one language generation metric or a specially designed metric, while the optimization reward can only optimize limited aspects. In order to boost generation performance more effectively, inverse reinforcement learning will also be taken into consideration to learn a more suitable reward for medical report generation in the future.
	

==> Experiments.tex <==
	
	\section{Experiments}
	

	
	
	\begin{table*}[ht] 
		
		\centering   
		\small
		\begin{tabular}{l|l|ccccccc}
			\hline  
			Dataset & Model & CIDEr & ROUGE-L  & METEOR & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4   \\ \hline 
			\multirow{6}{*}{\scriptsize{\textbf{IU X-Ray}}} 
			& top-down* & 0.206 & 0.334 & 0.144 & 0.279 & 0.178 & 0.119 & 0.079  \\ 
			&MRMA* &  0.325 & 0.309 & 0.163 & 0.382 & 0.252 & 0.173 & 0.120  \\ 
			&CACG & -- & \textbf{0.359} &--  & 0.369 & 0.246 & 0.171 & 0.115   \\ 
			\cline{2-9}   
			% & KER & 0.573 & 0.310 & 0.273 & 0.174 & 0.117 & 0.081 & -- \\
			% & KERP & \textbf{0.576} & 0.314 & 0.323 & 0.207 & 0.141 & 0.100 & \textbf{57.425}\\ 
			& MRG-X & 0.393 & 0.300 & 0.148 & 0.303 & 0.196 & 0.136 & 0.099  \\ 
			& ReMRG-X & \textbf{0.451} &0.346 & 0.180 & 0.391 & 0.262 & 0.184 & 0.131  \\ 
			& ReMRG-XR & 0.433 & \underline{0.357} & \textbf{0.184} & \textbf{0.402} & \textbf{0.276} &\textbf{ 0.196 }& \textbf{0.140}   \\ 
			%\hline
			\midrule 
			%\hline
			\multirow{6}{*}{\scriptsize{\textbf{MIMIC-CXR}}}  
			& top-down* & 0.359& 0.319& 0.134 & 0.233 & 0.159 & 0.119 & 0.093  \\ 
			&MRMA* & 0.324 & 0.330 & 0.157 & 0.361 & 0.244 & 0.182 & 0.141  \\
			&CACG & -- &0.307 & -- & 0.352 & 0.223 & 0.153 & 0.104  \\ 
			\cline{2-9}  
			& MRG-X & 0.383&0.323 & 0.156 & 0.345 & 0.231 & 0.170 & 0.131  \\ 
			& ReMRG-X & \textbf{0.415}&0.342 & 0.176 & 0.407 & 0.276 & 0.203 & 0.154  \\ 
			& ReMRG-XR & 0.411 & \textbf{0.342 }& \textbf{0.179} & \textbf{0.412} & \textbf{0.279} & \textbf{0.206 }& \textbf{0.157}  \\ 
			\hline 
		\end{tabular} 
		\caption{Automatic natural language evaluation on IU X-Ray (upper part) and MIMIC-CXR (lower part), compared with top-down~\protect\cite{anderson2018bottom}, 
			MRMA \cite{xue2018multimodal}, and 
			CACG \cite{liu2019clinically}, 
			* indicates our re-implementation. 	
		}
		%\vspace*{-1ex}
		\label{Table:report-generation} 
	\end{table*}
	
	
	
	
	\subsection{Datasets}
	
	%\subsubsection{IU X-Ray}
		In order to evaluate the performance of our proposed ReMRG-XR, extensive experiments have been conducted on the following two public chest x-ray image datasets.
		
	\smallskip \textbf{IU X-Ray} \cite{demner2016preparing} is a set of chest x-ray images with paired diagnostic reports collected by Indiana University. It contains 7,470 medical images and 3,955 corresponding reports, which mainly consists two sections: \textit{Impression} and \textit{Findings}. As there are some images or reports missing, %for our experiment, 
	we filtered out 6,222 images including both %views of
	frontal and lateral views, along with 3,111 paired reports.
	
	We take  \textit{Impression} and \textit{Findings} as our generation object and preprocess the texts by converting all words to lowercase. After that, we tokenize the reports, resulting in 2068 unique words in total. As most words occur rarely, we exclude tokens appearing less than 5 times and get 776 tokens.
	
	
	%\subsubsection{MIMIC-CXR}
\smallskip \textbf{MIMIC-CXR} \cite{johnson2019mimic} is the largest publicly available dataset of chest medical images with free-text radiology reports, which consists of 377,110 images along with 227,827 free-text  reports. Similarly, we filtered out 76,724 pairs of images combined of posteroanterior (PA) or anteroposterior (AP) view and lateral (LL) view with their reports, which consist of both \textit{Impression} and \textit{Findings}.
We then apply the same preprocessing and keep tokens with more than 5 occurrences, ending up with 2991 tokens overall. 

Finally, for both datasets, we randomly partition them by patients into training, validation, and testing with a  ratio of 7:1:2 and make sure that there is no overlap between the sets. Words excluded are replaced by the token of 'UNK'.
	
	
	
	
	\subsection{Evaluation Metrics}
	
	To evaluate the performance of our proposed model, we use several different automatic language generation metrics including BLEU \cite{papineni2002bleu}, METEOR \cite{banerjee2005meteor}, ROUGE-L \cite{lin2004rouge}, and CIDEr \cite{vedantam2015cider}. In particular, BLEU is a popular machine translation evaluation metric, which aims at measuring the ratio of correct matches of n-grams between generated sequences and the ground truth.
    To address some defects in BLEU, METEOR further considered the accuracy and recall based on the whole corpus.
    ROUGE-L is a metric for summary evaluation via measuring the longest common sequence that matches between two sequences based on recall. 
    Differently from the aforementioned metrics, CIDEr was designed especially for image description, which is most suitable for our task. It computes the term frequency inverse document frequency (TF-IDF) weight of n-grams to obtain the similarity between the candidate sequences and the reference sequences.
	
	
	
	\subsection{Implementation Details}
	We use  ResNet-101 pre-trained on ImageNet \cite{deng2009imagenet} to extract the region-level features, which are from the last convolutional layer. As both views of medical images are sent into the model simultaneously, two original 2048-dimensional region features are concatenated to a 4096-dimensional vector, which is later transformed into the visual embedding of size 1024.
	Next, four stacks of x-linear attention blocks are used to explore the high-order intra-modal interactions.
	During \textit{Decode}, we set the hidden layer size and word embedding dimension to 1024.
	As most reports are within a fixed length, we set the max generation length of IU X-Ray and MIMIC-CXR to 114 and 184, respectively.
	
	In training, we first pre-train the model with cross-entropy loss for 60 epochs with a batch size of 8 with NVIDIA RTX 2080 GPUs. Setting the base learning rate to  0.0001, we utilize the Noam decay strategy with 10,000 warmup steps with Adam \cite{kingma2014adam} as the optimizer.
	In the reinforcement learning stage, we select CIDEr as our training reward. We set the base learning rate to 0.00001 and decay with CosineAnnealing with a period of 15 epochs. We also set the maximum iteration to  60 epochs and the batch size to  2. We use beam search with a beam size of 2 for training.
	
	
	\begin{figure*}[!tb]
		%\vspace{-0.2in}
		\centering {\includegraphics[width=0.98\textwidth]{figures/sample.pdf}}
		%\vspace{-0.06in}
		\caption{Examples of reports generated by ReMRG-XP, ReMRG-X, MRG-X, MRMA, and Top-Down.}
		\label{fig:sample}
		%\vspace{-0.2in}
	\end{figure*}
	
	\subsection{Baseline Models}
	
	On both datasets, we compare our method with three state-of-the-art image captioning and medical report generation models: (i) CACG \cite{liu2019clinically}, which is the most similar work to ours, enhancing the capacity of the generation model with reinforcement learning,  
	(ii) our re-implementation of the top-down model \cite{anderson2018bottom}, which employs a conventional attention mechanism that calculates the contribution of regional features to the texts to be generated, and  
	(iii) MRMA \cite{xue2018multimodal}, in which reports are generated sentence by sentence with a recurrent way to generate long paragraphs. For our implemented methods, we use the same visual features and train/test split on both datasets.
	
	Additionally, we perform several ablation studies to inspect the effectiveness of different modules of our method. Specifically, we additionally implemented two simplified versions of our proposed ReMRG-XR by: 
	(i) first removing the repetition penalty from ReMRG-XR to  get a simplified model, called ReMRG-X, 
	and (ii) then removing both reinforcement learning and the repetition penalty to get another simplified model, called  MRG-X.
	
		\begin{figure*}[!tb]
		\centering
		
		\subfigure[BLEU-1]{
			\begin{minipage}[t]{0.32\linewidth}
				\centering
				\includegraphics[width=2.3in]{figures/bleu1_plot.pdf}
				%\caption{fig1}
			\end{minipage}%
		}%
		\subfigure[BLEU-4]{
			\begin{minipage}[t]{0.32\linewidth}
				\centering
				\includegraphics[width=2.3in]{figures/bleu4_plot.pdf}
				%\caption{fig2}
			\end{minipage}%
		}%
		\subfigure[CIDEr]{
			\begin{minipage}[t]{0.32\linewidth}
				\centering
				\includegraphics[width=2.3in]{figures/cider_plot.pdf}
				%\caption{fig2}
			\end{minipage}
		}%
		
		\subfigure[METEOR]{
			\begin{minipage}[t]{0.32\linewidth}
				\centering
				\includegraphics[width=2.3in]{figures/meteor_plot.pdf}
				%\caption{fig2}
			\end{minipage}
		}%
		\subfigure[ROUGE-L]{
			\begin{minipage}[t]{0.32\linewidth}
				\centering
				\includegraphics[width=2.3in]{figures/rouge_plot.pdf}
				%\caption{fig2}
			\end{minipage}
		}%
		\subfigure[Learning Rate]{
			\begin{minipage}[t]{0.32\linewidth}
				\centering
				\includegraphics[width=2.3in]{figures/lr_plot.pdf}
				%\caption{fig2}
			\end{minipage}
		}%
		\centering
		\caption{ Results of medical report generation in times of different learning rate decay strategies}
		\label{fig:lr}\vspace*{-1ex}
	\end{figure*}
	
	
%	\subsection{Results and Analysis}
	
%	We now first compare our ReMRG-XR method with several state-of-the-art methods. Then, we validate the effectiveness of the fundamental components of our model, including x-linear attention,  reinforcement learning, and repetition penalty. We then further evaluate the influence of network parameters, such as the strategy of learning rate decay.
	
	

	
	
\subsubsection{Main Results.}
Table~\ref{Table:report-generation} shows the experimental results of the proposed ReMRG-XP, two simplified versions (ReMRG-X and MRG-X), and three baselines in terms of seven natural language generation metrics, where two of the baselines are re-implemented by ourselves (denoted by *). In addition, Figure~\ref{fig:sample} exhibits some examples of reports generated by these methods.
Generally, ReMRG-XP greatly outperforms all state-of-the-art baselines in all metrics  in Table~\ref{Table:report-generation}, and as in Figure~\ref{fig:sample}, it also generates more coherent and accurate report than the baselines. This finding proves the effectiveness of ReMRG-XP.
Furthermore, The performance of ReMRG-X is generally worse than ReMRG-XP, except for CIDEr. This is because ReMRG-X uses CIDEr as reward which is fragile with generating repeated terms, while repetition penalty is used in ReMRG-XP to overcome this problem, making it capable of generating more coherent and readable descriptions. This observation is also well supported by the report examples in Figure~\ref{fig:sample}. 
Comparing to ReMRG-X and ReMRG-XP, the performance of MRG-X is not very satisfactory because reinforcement learning is not utilized in MRG-X. However, MRG-X still significantly outperforms the top-down baseline, proving the effectiveness of using x-linear attention to obtain higher order features.	
	
	
	%The results evaluated on seven natural language generation metrics have been shown in Table~\ref{Table:report-generation}.
	%For comparison, we choose three baseline models for medical report generation, where two of which are our re-implementation. 

	%As shown in Table~\ref{Table:report-generation}, ReMRG-XP and its simplified models both outperform the state-of-the-art baselines in CIDEr. Though other scores of MRG-X may not have apparent advantages above baselines, they have a large boost after training with reinforcement learning. With our repetition penalty module integrated, our proposed ReMRG-XR achieves generally much better performances than all baselines in terms of all metrics on both datasets.
	
	%As observed from Figure~\ref{fig:sample}, all of our versions of models could match more terms compared with the baselines especially ReMRG-X and ReMRG-XR, which demonstrates the effectiveness of our x-linear attention and reinforcement learning. With reinforcement learning added, we can see that the matched terms increase while the global coherency is still mssing. To alleviate this problem, repetition penalty is integrated and the qualitative results prove that our proposed ReMRG-XR can generate more coherent reports with high accuracy.
	
	%Fig~3 demonstrates the qualitative results of our proposed models and baseline models. From which we can have following observations: firstly, baselines can match few terms while poor in coherent. Secondly, the proposed MRG-X can match more terms compare to baselines but still has poor continuity. ReMRG-XP and its simplified model not only can match more terms, but also have better consistency in sentences which make the generated medical imaging reports more readable. 
	
	
	%In particular, on IU X-Ray dataset, our encoder-decoder model achieved almost twice as well as that of the state-of-the-art result. Since CIDEr is specially designed for image description, the significant improvements have demonstrated the efficacy of our method.
	
	% Moreover, although the CIDEr score drops a little when finetuning with reinforcement learning on IU X-Ray, the performance of other evaluation metrics all raise a lot, which may contribute to the limit of the size of the dataset.  In addition, the ablation study also shows that with diversity considered, our model tend to generate more qualified reports.
	
	\subsubsection{Effectiveness of X-Linear Attention.}
In this subsection, we use top-down and CACG as the baselines to further the effectiveness of x-linear attention, because they are equivalent to MRG-X and ReMRG-X if their attention mechanisms are replaced by x-linear attention.
As shown in Table~\ref{Table:report-generation} ReMRG-X (resp. MRG-X) dramatically outperforms CACG (resp. top-down) in terms of all metrics, this is because x-linear attention can explore high-order feature interactions and achieve multi-modal reasoning, making it possible to generate more accurate reports.
Examples in Figure~\ref{fig:sample} tell the same story: the description generated by  MRG-X is more accurate (i.e., have more correctly matched terms) than that generated by top-down.



%	As introduced before, a key component of our model is x-linear attention.
%	In this group of experiments, we take top-down and CACG as our baselines, which adopt a top-down attention and SCST algorithm respectively. 
	%In this group of experiments, we take top-down as our baseline, which adopt top-down attention mechanism.
%	Comparing our MRG-X and top-down, and compare ReMRG-X and CACG, both results show that our poposed MRG-X and ReMRG-X outperform the baselines on almost all metrics especially on CIDEr.
% Since CIDEr gives a higher importance to key phrases, the boost on CIDEr has proved the effectiveness of our MRG-X to describe more informative phrases. 
	%Since CIDEr is specially designed for image description, the significant improvements have demonstrated the efficacy of our method. 
%	Significant improvements have demonstrated the effectiveness of our x-linear attention, which can also be observed from Figure~\ref{fig:sample}. From Figure~\ref{fig:sample} we can observe that both our MRG-X and ReMRG-X match more terms compared with top-down, which demonstrate the accuracy of our x-linear module.
	

	
	
	\subsubsection{Effectiveness of Reinforcement Learning.}
	
	In this subsection, top-down and MRG-X are used as the baselines to further evaluate the effectiveness of reinforcement learning, because they are equivalent to CACG and ReMRG-X if reinforcement learning is introduced to them.
As shown in Table~\ref{Table:report-generation} ReMRG-X (resp. CACG) achieves much better performances than MRG-X (resp. top-down) in terms of all metrics. Similarly, the example report of ReMRG-X in Figure~\ref{fig:sample} is also more accurate and readable than that generated by MRG-X.
These findings both demonstrate that by applying reinforcement learning, medical report generation models can achieve much better performances.
	
%	Since only the CIDEr metric has raised a lot with our x-linear attention,
%	to make the improvements more comprehensive, reinforcement learning is utilized to boost performance. In this group of experiments, we compare our ReMRG-X model with MRG-X.
%	As illustrated in Table~\ref{Table:report-generation}, the performance of our ReMRG-X outperforms MRG-X in terms of all metrics. Similar results can be seen comparing CACG and top-down, which demonstrate the effectiveness and robustness of fine-tuning with reinforcement learning for medical report generation.
	
%	As observed from Figure~\ref{fig:sample}, both the matched terms and the global coherency increase with reinforcement learning finetuned.
	
	\subsubsection{Effectiveness of Repetition Penalty.}
	
	
Though our proposed ReMRG-X has achieved significant improvements especially on CIDEr, performance on other metrics that focus more on the global fluency of generated reports has not outperformed the baselines a lot.
In order to generate more coherent descriptions and raise the readability, 
we utilize repetition penalty into greedy search during reinforcement learning. In this group of experiments, we use ReMRG-X as baseline to verify the effectiveness of repetition penalty.
Results in Table\ref{Table:report-generation} show that our proposed ReMRG-XR outperforms ReMRG-X on almost all metrics except CIDEr.
Since CIDEr lays more weight on the significant phrases, while the other metrics give more importance to the global fluency, improvements on other metrics demonstrate the effectiveness of the repetition penalty module to generate more coherent and readable sentences. 
Considering the CIDEr scores are significantly high, we believe it is worth of slightly sacrificing CIDEr to obtain significant improvements in other metrics, and to enhance the overall readability of the report.
Examples in Figure~\ref{fig:sample} also demonstrate that our ReMRG-XR can generate more coherent sentences compared with ReMRG-X while keeping high accuracy. 

	
	
	%Especially, the performance on IU X-ray boosts a little bit more, which %declares 
	%shows that the repetition penalty contributes more to small datasets.
	
	\subsubsection{Influence of Learning Rate Decay.}
	
We also investigate the influence of the strategy of learning rate decay when training with reinforcement learning by comparing the performances using \textit{Plateau} and \textit{CosineAnnealing} strategies, and the experimental results are presented in Figure~\ref{fig:lr}.
We train on IU X-ray for 70 epochs with a batch size of two. The initial learning rate is all set to 0.00001. For \textit{Plateau} strategy, the learning rate is reduced by a factor of 0.8, once learning stagnates for 3 epochs. For the CosineAnnealing strategy, the cosine function is used as the learning rate annealing function, the maximum number of iteration epoch is set to be 10, and the minimum learning rate is $\rm{4e^{-8}}$. From Figure~\ref{fig:lr}, we can observe that all evaluation scores using CosineAnnealing are beyond that using the Plateau decay strategy, and when the scores of Plateau have achieved their highest points, the scores of CosineAnnealing still keep increasing. Thus, we apply the CosineAnnealing learning rate decay strategy during reinforcement learning in our work.
	
%	\section{Discussion}
	
%	In this section, we first summarize the main differences between our proposed ReMRG-XR method and other state-of-the-art works for medical report generation. % We also point out the limitations of our work as well as the potential solutions to address these limitations in the future.
	
%	\subsection{Comparison with Previous Works}
	
%	Compared with conventional encoder-decoder architecture for medical report generation, our proposed ReMRG-XR further boosts the generation performance by reinforcement learning. We also utilize repetition penalty into reinforcement learning to make the generated reports more diverse.
	
%	Our work is also different from previous works exploring first-order feature interactions, our method further explored high-order inter-modal and intra-modal interactions, which is more capable of single-modal and multi-modal reasoning. Significant improvements have been demonstrated in the evaluated results.
	
	
%	\subsection{Limitations and Future Work}
%	While our ReMRG-XR method for medical report generation has achieved a superior performance compared to other state-of-the-art works, its performance could be further improved in the future by dealing with the following limitations and challenges.
	
%	\textit{Firstly}, while our generated reports are generally satisfactory according to Figure~\ref{fig:sample}, our reports tend to generate normal descriptions according to the unbalance of the datasets. Considering the similarity of the normal descriptions, we could potentially divide the sentences to be generated into normal and abnormal and pay more attention to the generation of abnormal sentences.
	
%	\textit{Secondly}, Since no effective metrics have been specially designed for medical report generation, and the evaluation of the generated results rely on human evaluation to a large extent.
%	In order to evaluate our generated results more effectively, we will explore a more reasonable and effective metric
%	for medical report generation in future work. 
	
%	\textit{Thirdly}, Most current works utilizing reinforcement learning only optimize one language generation metric or a specially designed metric, while the optimization reward can only optimize limited aspects. In order to boost generation performance more effectively, inverse reinforcement learning will also be taken into consideration to learn a more suitable reward for medical report generation.

==> Methods.tex <==

	
	\section{Methods}
	
		\begin{figure*}[!tb]
		%\vspace{-0.2in}
		\centering {\includegraphics[width=0.98\textwidth]{figures/framework.pdf}}
		%\vspace{-0.06in}
		\caption{The architecture of our proposed ReMRG-XR network. 
			%ResNet-101 is firstly utilized to extract global and regional features. After that, features from different views are concatenated accordingly. Next, we utilize a stack of x-linear attention blocks in the visual encoder to encode the visual features with the higher-order intra-modal interactions to enhance our extracted features. Then the attended image features are sent into the sentence decoder, along with the x-linear attention blocks, to enhance the multi-modal reasoning. Finally, after pretraining with the Encoder-Decoder architecture, our model is finetuned via RL with diversity considered.
		}\vspace*{-1ex}
		\label{fig:framework}
		%\vspace{-0.2in}
	\end{figure*}
	
	
	
%	In this paper, we choose to generate the \textit{Impression} and the \textit{Findings} section. To learn high order feature interactions both spatially and channel-wise, we introduce an x-linear attention based network and finetune it with RL. In the following, we will detail our network design and implementation details for medical report generation.
	
	
	We propose a reinforced medical report generation method with x-linear attention and repetition penalty (ReMRG-XR). Intuitively, we believe that the use of high-order feature interactions will strengthen the model's capacity in single- and multi-modal reasoning, which will enhance the model's performance in terms of accuracy of the generated reports. Besides, we consider that the combination of the integrated penalty with the repetition term will produce much more diverse sentences, which will increase the coherency and readability of the generated diagnosis reports.  
	
	Specifically, as shown in Figure~\ref{fig:framework}, to improve the clinical accuracy of the generated reports, 
	we take the global visual features extracted from medical images $f_{global}$ as input \textbf{Q} and the regional features $f$ as input \textbf{V} and \textbf{K}. A stack of x-linear attention blocks are used to calculate the outer product between two feature vectors and enable  channel-wise attention through the squeeze-excitation operation. As such, high-order intra-modal feature interactions are explored during the encoder procedure. 
	After that, the embedded attended features $\hat{f}$ are combined and sent into LSTMs during the decoder procedure. The output hidden state of the LSTMs together with the final attended visual features are then sent into an x-linear attention block to explore multi-modal feature interactions, which is later used for word prediction.
	After pretraining with such an encoder-decoder architecture for epochs, reinforcement learning is used to boost the performance, during which we employ the SCST algorithm and set CIDEr as the reward. To generate more readable descriptions, we use a repetition penalty in SCST to increase the readability of the generated reports.
	
		
	\begin{table}[!tb]
		
		\centering
		\begin{tabular}{c|c}
			
			\toprule
			Symbol & Explanation\\
			\midrule
			%\midrule
			$f_{global}$ & global averaged visual features \\
			${X}^k_i$ & the joint bi-linear representation of query-key \\
			${X}^k_v$ & the joint bi-linear representation of query-value \\
			$a^s$ & spacial attention weights \\
			$A^s$ & spacial attention distribution \\
			$\bar{X}$ & channel-wise descriptor \\
			$A^c$ & channel-wise attention distribution \\
			$a^c$ & channel-wise attention weights \\
			$\hat{f}$ &x-linear attended features \\
			\bottomrule
		\end{tabular}
		\caption{Frequently Used Symbols}
		\label{tab:formla1}\vspace{-2ex}
	\end{table}
	
	
	\subsection{Encoder-Decoder Framework}
	\subsubsection{Visual Encoder.}
	In our work, a ResNet-101-based network pre-trained on ImageNet is employed to extract the global and regional visual features of the different views (frontal and lateral) of a patient's chest x-rays. We resize our input images to 224$\times$224 to keep them consistent with our pre-trained ResNet-based CNN encoder. Then, the regional features $f\in \mathbb{R}^{2048 \times 196}$ (reshaped from 2048$\times$14$\times$14) are extracted from the last convolutional layer of ResNet-101, which represents 196 sub-regions. A global average pooling is applied to the extracted regional features to obtain the global features $f_{global}$. After that, both global and regional features are concatenated according to different views before feeding into the next layers. In this paper, we choose to generate the \textit{Impression} and the \textit{Findings} section. To learn high-order feature interactions both spatially and channel-wise, we introduce an x-linear-attention-based network and fine-tune it with reinforcement learning. In the following, we will detail our network design and implementation details for medical report generation.
	
	
	To enhance the visual features obtained above, we employ a stack of x-linear attention blocks, which is capable of catching high-order feature interactions.
	Taking the combined regional features $f$ as the initial input keys  ${\bf{K}}=\{{\bf{k}}_i\}_{i=1}^N$ and the values  ${\bf{V}}=\{{\bf{v}}_i\}_{i=1}^N$, and the global features $f_{global}$ as the initial input query $\textbf{Q}$, we attend the input features with our x-linear attention as in Figure~\ref{fig.attention}.
	

	
	Bi-linear pooling is first used for fine-grained image classification. It has recently been applied to multi-modal feature fusion in visual question answering, aiming at exploring multi-modal interactions. We use it in our medical report generation to explore high-order intra-modal interactions in medical image features and inter-modal interactions between the radiograph features and the respective reports.
	First, we do a low-rank bi-linear pooling  \cite{kim2018bilinear} on both the input query and key, and the query and values to get the joint bi-linear representation of query-key $\textbf{X}^k_i$ and query-value $\textbf{X}^v_i$, which encodes the second-order feature interactions of query-key and query-value.
	
	
	Next, we transform the query-key representations $\textbf{X}^k_i$ into query-key representations $\textbf{X}^{'k}_i$ with an embedding layer. Both spacial and channel-wise bi-linear attention distributions are obtained according to the transformed query-key representations $\textbf{X}^{'k}_i$. Specifically, we perform a spatial attention via another embedding layer to obtain the spacial attention weights $ a^s$, and normalize it with a softmax layer to get the spatial attention distribution ${\bm{A}}^s$.  Meanwhile, the channel-wise attention is achieved via a squeeze and excitation operation \cite{hu2018squeeze}, in which the squeeze performs a global average pooling to obtain a global channel-wise descriptor $\bar{\bf{X}}$, and the excitation produces the channel-wise attention distribution ${\bm{A}}^c$  with the gating mechanism via a fully connected (FC) layer along with a sigmoid.
	
	Finally, we generate the x-linear-attended features $\hat{f}$ by computing the spatial and channel-wise weighted bi-linear feature representation.
	
	
	\begin{figure}
		%\vspace{-0.1in}
		\centering {\includegraphics[width=0.475\textwidth]{figures/attention.pdf}}
		%\vspace{-0.06in}
		\caption{x-linear Attention Block}
		\label{fig.attention}\vspace*{-1ex}
		%\vspace{-0.2in}
	\end{figure}
	
	
	\begin{equation}\label{Eq:Eq1}\small
	{\bf{X}}^k_i=\sigma\left({W}_k{{\bf{k}}_i}\right) \odot \sigma\left({W}^k_q{\bf{Q}}\right),
	\end{equation}
	\begin{equation}\label{Eq:Eq2}\small
	{\bf{X}}^v_i=\sigma\left({W}_v{{\bf{v}}_i}\right) \odot \sigma\left({W}^v_q{\bf{Q}}\right),
	\end{equation}
	
	\begin{equation}\label{Eq:Eq3}\small
	{\bf{X}}^{'k}_i = \delta\left({W}^k_x{\bf{X}}^k_i\right),
	\end{equation}
	\begin{equation}\label{Eq:Eq4}\small
	a^s_{i}={W}_s{\bf{X}}^{'k}_i, {\bm{A}}^s=softmax\left({\bf{a}}^s\right),
	\end{equation}
	\begin{equation}\label{Eq:Eq5}\small
	\bar{\bf{X}}={1 \over N}\sum\nolimits_{i = 1}^N {{\bf{X}}^{'k}_i}.
	\end{equation}
	\begin{equation}\label{Eq:Eq6}\small
	{\bf{a}}^c={W}_e \bar{\bf{X}},{\bm{A}}^c=sigmoid\left(\bf{a}^c\right),
	\end{equation}
	\begin{equation}\label{Eq:Eq7}\small
	\begin{array}{l}
	\hat{f}=Attention\left({\bf{K}}, {\bf{V}}, {\bf{Q}}\right)={\bm{A}}^c\odot\sum\nolimits_{i = 1}^N {{a}_i^s{{\bf{X}}^v_i}},
	\end{array}
	\end{equation}
	where ${W}_k$,  ${W}_v$, ${W}_q^k $, ${W}_q^v$, ${W}_x^k$, ${W}_s $, ${W}_e $     are embedding matrices, $\sigma$ denotes an \textbf{ELU} unit, $\delta$ denotes a  \textbf{ReLU} unit, and $\odot$ represents element-wise multiplication.
	
	In order to extend to higher-order intra-modal feature interactions, our visual encoder is composed of a stack of x-linear attention blocks. 
	Specifically, we take the previous output x-linear attended feature  $\hat{f}^{(n-1)}$ as input query Q, along with the current keys ${\bf{K}}^{(n-1)}=\{{\bf{k}}_i^{(n-1)}\}_{i=1}^N$ and values ${\bf{V}}^{(n-1)}=\{{\bf{v}}_i^{(n-1)}\}_{i=1}^N$, which are updated through concatenating with the new attended feature via a residual connection and layer normalization.
	
	\begin{equation}\label{Eq:Eq8-1}\small
	\hat{f}^{(n)}=Attention\left( {\bf{K}}^{(n-1)}, {\bf{V}}^{(n-1)}, \hat{f}^{(n-1)}\right),
	\end{equation}
	\begin{equation}\label{Eq:Eq8-2}\small
	{\bf{k}}_i^{(n)}=LN(\sigma({W}^k_n[\hat{f}^{(n)},{\bf{k}}_i^{(n-1)}])+{\bf{k}}_i^{(n-1)}),
	\end{equation}
	
	\begin{equation}\label{Eq:Eq8-3}\small
	{\bf{v}}_i^{(n)}=LN(\sigma({W}^v_n[\hat{f}^{(n)},{\bf{v}}_i^{(n-1)}])+{\bf{v}}_i^{(n-1)}),
	\end{equation}
	where $W^v_n$ and $W^k_n$ are embedding matrices, $\bf{v}_i^{(n)}$ and $\bf{k}_i^{(n)}$ represents the $i^{th}$ key/value, $\sigma$ denotes a \textbf{ReLU} unit, 
	and $LN$ denotes layer normalization operation. We repeat this process for 4 times to achieve $8^{th}$-order feature interactions.
	
	\subsubsection{Sentence Decoder.}
	The sentence decoder takes the combination of different order attended region-level visual features $\hat{f}^{(n+1)}$ and the global image feature $f_{global}$ as input $\tilde{f}$ , and generates the report word by word. In order to exploit high order inter-modal interactions between visual features and semantic features, we employ an x-linear attention-based LSTM decoder. 
	
	\begin{equation}\label{Eq:Eq9}\small
	\tilde{f}={\rm{W}}_c[\hat{f}^{(0)},\hat{f}^{(1)},...,\hat{f}^{(1+N)}],
	\end{equation}
	
	\begin{equation}\label{Eq:Eq10}\small
	h_t = LSTM(\tilde{f}; w_{t}, h_{t-1}, c_{t-1})
	\end{equation}
	where ${\rm{W}}_c$ is an embedding matrix,  $\hat{f}^{(0)} = f_{global}$,  $w_{t}$ is the current input word, $h_{t-1}$ is the previous LSTM hidden state, and $c_{t-1}$ is the previous context vector. Next, we take the output hidden state $h_t$ of the LSTM as the input query \textbf{Q} of x-linear attention block, and the final output attended feature $f^{(N+1)}$ from the visual encoder as keys \textbf{K} and values \textbf{V}.
	
	\begin{equation}\label{Eq:Eq11}\small
	\hat{f}_d=Attention\left({\bf{K}}, {\bf{V}}, {\bf{Q}}\right)=Attention\left({f^{(N+1)}}, {f^{(N+1)}}, {h_t}\right).
	\end{equation}
	
	After that, we compute the current context vector $c_t$ with a residual connection and a gated linear unit (GLU), followed by a fully connected layer. 
	
	\begin{equation}\label{Eq:Eq12}\small
	c_t = {\rm{W}}_c(\sigma (h_t + {\rm{W}}_L(h_t+\hat{f}_d))),
	\end{equation}
	where ${\rm{W}}_c$ and  ${\rm{W}}_L$   are embedding matrices, and $\sigma$ denotes a \textbf{GLU} unit. Finally, the context vector $c_t$ is sent into a softmax layer to predict the next word $w_{t+1}$.  
	
	\begin{equation}\label{Eq:Eq13}\small
	w_{t+1} = Softmax(c_t)
	\end{equation}

	
	
	\subsection{Reinforcement Learning for Diversity.}
	The reinforcement learning algorithm commonly used in existing medical report generation %methods 
	\cite{10.1007/978-3-030-32692-0_77,liu2019clinically} is the self-critical sequence training (SCST) algorithm \cite{rennie2017self}, which directly optimizes the automatic natural language generation (NLG) metrics. Since most of the existing works employing SCST take CIDEr  \cite{vedantam2015cider} as the reward, which focuses on phrase-level accuracy, ignoring the global fluency and diversity, we consider diversity-based~SCST with repetition penalty integrated.
	
	SCST adopts a policy gradient method to optimize a non-differentiable metric such as CIDEr. In order to normalize the reward and reduce the variance during training, SCST utilizes the REINFORCE algorithm with a baseline, which is obtained from the inference reward by greedy search. The goal is to minimize the negative expected reward.
	The final gradient of the optimization object is:
	
	\begin{equation}\label{Eq:Eq14}\small
	\frac{\partial{L(\theta)}}{\partial{s_t}} = (r(w^s) - r(\hat{w}))\bigtriangledown_{\theta}\log p_{\theta}(w^s | x), 
	\end{equation}
	where $w^s  = (w_1^s, . . . ,w_T^s )$ is a Monte-Carlo sample from~$p_{\theta}$, $p_{\theta}$ is our generation model,  $r(w^s)$ is the current reward, and $r(\hat{w})$ is the reward obtained by the inference algorithm. 
	
	In order to decrease the probability of repeated terms generated in the reports,
	we thus introduce a penalty that would constraint the probabilities of words resulting in repeated trigrams. Specifically, we update the log-probability of the output word by subtracting a value proportional to the number of times the trigram has been generated.
	
	\begin{equation}
	p_w = p_w - n_w \times \alpha, 
	\end{equation}
	where $p_w$ is the log-probability of the word $w$, $n_w$ is the number of times the trigram has generated the word $w$, and $\alpha$ is a hyperparameter. In our work, we set $\alpha$ to 2. We employ this update mechanism during our greedy search process in SCST in order to generate more diverse paragraphs, thus avoiding the repetition problem.


==> RelatedWork.tex <==
		\section{Related Work}
	
	
%	\subsubsection{Deep-Learning-Based Medical Report Generation.}~Most %
%Deep learning-based methods utilize CNN to extract image features and feed them into LSTM to generate sequences. 
Most medical report generation approaches adopt encoder-decoder-based frameworks, which utilize CNNs as an encoder to extract image features and feed them into an RNN-based decoder to generate sequences. Recent works have been trying to explore more interactions between images and sentences via attention mechanisms  \cite{10.1007/978-3-030-26763-6_66,Wang_2018,jing-etal-2018-automatic,xue2018multimodal}. \citet{jing-etal-2018-automatic} propose a co-attention mechanism that builds attention distributions separately for visual and semantic domains and ignores multi-modal interactions. \citet{xue2018multimodal} develop a sentence-level attention mechanism to explore multi-modal interactions, which compute the attention distribution over visual regions according to sentence-level semantic features. 
	However, all these methods solely explore first-order feature interactions; differently, in this work, both intra-model and inter-modal high-order feature interactions are explored by x-linear attention, and reinforcement learning is further used to enhance the model's performance. 
	
	%However, most of them have been focusing on the first-order interaction between visual features and semantic features leading to the limited capacity of reasoning high order interactions, especially for the complexity of medical images. Recently, \cite{Pan2020} proposed an x-linear attention mechanism which is capable of exploiting high order feature interactions for image captioning via low-rank bilinear pooling, while such bilinear pooling-based methods haven't been introduced to the medical domain.
	%However, most of these methods encounter the challenges of inconsistent training goals and exposure bias, which motivate us to employ reinforcement learning to address the aforementioned challenges.
	
%	\subsubsection{Reinforcement Learning Based Medical Report Generation}
	%While deep learning-based methods have achieved good results, it's still far from satisfactory according to the exposure bias and non-differentiable metrics.
	%Compositional architecture-based methods are composed of other independent blocks. 
	%Since the effectiveness of reinforcement learning have been proved by recent works, 
	With  rapid advances in reinforcement learning,
	many efforts have used reinforcement learning for automatic medical report generation to boost the performance \cite{10.1007/978-3-030-32692-0_77,liu2019clinically,li2018hybrid}. Specifically, \citet{li2018hybrid} propose a hybrid retrieval-based model with reinforcement learning to determine whether to generate a sentence via template retrieval or LSTMs. Subsequently,  \citet{10.1007/978-3-030-32692-0_77} and  \citet{liu2019clinically} adopt reinforcement learning to directly optimize the text generation.
	Compared to existing reinforcement learning solutions, the proposed ReMRG-XR have two advantages: (i) it uses x-linear attention blocks to enhance the model's capability in exploring high-order feature interactions and multi-modal reasoning, and (ii) a repetition penalty is introduced to make the model generate more diverse and coherent long sentences.
	%Recently, some works began to use reinforcement learning-based methods that combine template-based approaches with traditional generative models for medical report generation. \cite{li2018hybrid} proposed a hybrid retrieval-based model with reinforcement learning to select whether to generate a sentence via retrieving a template or LSTM. Since the effectiveness of reinforcement learning have been proved by recent works, several works have employed reinforcement learning for automatic report generation to boost the performance \cite{10.1007/978-3-030-32692-0_77,liu2019clinically}.
	%While according to the complexity of the long paragraph, simple REINFORCE with a baseline they utilized cannot handle such long sequences. 
	%Since the sentences generated by reinforcement learning tend to be lack of diversity, we are motivated to raise the readability and diversity of generated reports by employing repetition penalty during reinforcement learning.
	
%	\subsubsection{Image Captioning}
	Image captioning is a similar task to medical report generation. \citet{anderson2018bottom} first introduce Faster R-CNN to image captioning to extract the features of the region of interest. \citet{lu2017knowing} propose an adaptive attention mechanism to determine whether to pay attention to the corresponding images when predicting the next word for image caption generation.
	Similarly to our work, \citet{Pan2020} also use a x-linear attention mechanism to generate more accurate captions for natural images.
	%Recently, \cite{Pan2020} proposed bi-linear pooling-based  attention to exploit high order feature interactions, which inspire us to introduce such bi-linear pooling based attention to our work. 
	Similarly,   \citet{melas2018training} also introduce a penalty mechanism when generating captions to reduce the occurrence of recurring terms.
  Differently from these works, this paper focuses on the task of medical report generation, which is more challenging than the image captioning task. 
	First, medical images often have noise or artifacts, making them more difficult to learn than data used in image captioning.
	Second, medical image reports have to describe medical-related objects and conditions, so the generated textual descriptions in medical report generation request higher professionalism and accuracy than those in image captioning.
	Third, image captioning solely needs to generate short descriptions regarding the corresponding images, while the medical report generation task not only needs to generate much longer descriptions, but also has to summarize the information of medical images, give a professional diagnosis (e.g., normal or abnormal), and describe the specific information of the interested objects (e.g., the locations and sizes of lesions).
	
	
	%\red{
	%First, the targets of image captioning are common things in daily life, while those of medical report generation are complex medical lesions.
	%Second, according to the high complexity of medical images, slight differences in medical images can contribute to great changes in corresponding reports. 
  %Third, differently from image captioning, medical report generation requires long and coherent paragraphs, which demands more on readability.}
	
	%Since medical report generation aims to generate detailed paragraphs, when applying standard image caption methods to generating long sequences, challenges remain for generating diverse sentences. \cite{melas2018training} proposed to integrate repetition penalty to raise the diversity for image caption while such methods haven't been introduced to medical report generation. 
	
	%Though image caption is similar to our task to some extent, medical report generation is more complex according to the poor quality of medical images and the high demand for description. In order to generate reports more comprehensively, we propose to employ x-linear attention and repetition penalty in our medical report generation.
	%Inspired by the aforementioned works, we further integrate the x-linear attention mechanism to our task and enhance the automatic medical report generation via RL with diversity added.
	

